PASTA: Controllable Part-Aware Shape Generation with Autoregressive Transformers

The increased demand for tools that automate the 3D content creation process led to tremendous progress in deep generative models that can generate diverse 3D objects of high fidelity. In this paper, we present PASTA, an autoregressive transformer architecture for generating high quality 3D shapes. PASTA comprises two main components: An autoregressive transformer that generates objects as a sequence of cuboidal primitives and a blending network, implemented with a transformer decoder that composes the sequences of cuboids and synthesizes high quality meshes for each object. Our model is trained in two stages: First we train our autoregressive generative model using only annotated cuboidal parts as supervision and next, we train our blending network using explicit 3D supervision, in the form of watertight meshes. Evaluations on various ShapeNet objects showcase the ability of our model to perform shape generation from diverse inputs \eg from scratch, from a partial object, from text and images, as well size-guided generation, by explicitly conditioning on a bounding box that defines the object's boundaries. Moreover, as our model considers the underlying part-based structure of a 3D object, we are able to select a specific part and produce shapes with meaningful variations of this part. As evidenced by our experiments, our model generates 3D shapes that are both more realistic and diverse than existing part-based and non part-based methods, while at the same time is simpler to implement and train.

==> fig/shape_completion_diversity_fixed_root.tex <==
\begin{figure}
    \centering
    \vspace{-1.2em}
    \begin{subfigure}[b]{0.25\linewidth}
		\centering
        Partial Input
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[b]{0.75\linewidth}
		\centering
        Object Completions
    \end{subfigure}%
    \vskip\baselineskip%
    \vspace{-1.5em}
    \begin{subfigure}[b]{0.25\linewidth}
		\centering
		\includegraphics[width=\linewidth]{shape_variation_fixed_root/chairs/starting/36976_2.png}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[b]{0.25\linewidth}
		\centering
		\includegraphics[width=\linewidth]{shape_variation_fixed_root/chairs/completed/36976_16_2.png}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[b]{0.25\linewidth}
		\centering
		\includegraphics[width=\linewidth]{shape_variation_fixed_root/chairs/completed/36976_16.png}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[b]{0.25\linewidth}
		\centering
		\includegraphics[width=\linewidth]{shape_variation_fixed_root/chairs/completed/36976_18.png}
    \end{subfigure}%
    \vskip\baselineskip%
    \vspace{-2.5em}
    \begin{subfigure}[b]{0.25\linewidth}
		\centering
		\includegraphics[width=\linewidth]{shape_variation/chairs/starting/37079_4.png}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[b]{0.25\linewidth}
		\centering
		\includegraphics[width=\linewidth]{shape_variation/chairs/completed/37079_22.png}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[b]{0.25\linewidth}
		\centering
		\includegraphics[width=\linewidth]{shape_variation/chairs/completed/37079_23.png}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[b]{0.25\linewidth}
		\centering
		\includegraphics[width=\linewidth]{shape_variation/chairs/completed/37079_23_2.png}
    \end{subfigure}%
    \vskip\baselineskip%
        \vspace{-3.2em}
    \begin{subfigure}[b]{0.25\linewidth}
		\centering
		\includegraphics[width=\linewidth]{shape_variation/tables/starting/22763_1.png}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[b]{0.25\linewidth}
		\centering
		\includegraphics[width=\linewidth]{shape_variation/tables/completed/22763_10.png}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[b]{0.25\linewidth}
		\centering
		\includegraphics[width=\linewidth]{shape_variation/tables/completed/22763_10_2.png}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[b]{0.25\linewidth}
		\centering
		\includegraphics[width=\linewidth]{shape_variation/tables/completed/22763_10_3.png}
    \end{subfigure}%
    \vskip\baselineskip%
    \vspace{-3.2em}
    \begin{subfigure}[b]{0.25\linewidth}
		\centering
		\includegraphics[width=\linewidth]{shape_variation/tables/starting/21168_3.png}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[b]{0.25\linewidth}
		\centering
		\includegraphics[width=\linewidth]{shape_variation/tables/completed/21168_9.png}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[b]{0.25\linewidth}
		\centering
		\includegraphics[width=\linewidth]{shape_variation/tables/completed/21168_11.png}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[b]{0.25\linewidth}
		\centering
		\includegraphics[width=\linewidth]{shape_variation/tables/completed/21168_12.png}
    \end{subfigure}%
    \vskip\baselineskip%
    \vspace{-2.5em}
    \begin{subfigure}[b]{0.25\linewidth}
		\centering
		\includegraphics[width=\linewidth]{shape_variation/lamps/starting/14250_4.png}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[b]{0.25\linewidth}
		\centering
		\includegraphics[width=\linewidth]{shape_variation/lamps/completed/14250_8.png}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[b]{0.25\linewidth}
		\centering
		\includegraphics[width=\linewidth]{shape_variation/lamps/completed/14250_9_2.png}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[b]{0.25\linewidth}
		\centering
		\includegraphics[width=\linewidth]{shape_variation/lamps/completed/14250_9_4.png}
    \end{subfigure}%
    \vskip\baselineskip%
    \vspace{-2.5em}
    \begin{subfigure}[b]{0.25\linewidth}
		\centering
		\includegraphics[width=\linewidth]{shape_variation/lamps/starting/14231_1.png}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[b]{0.25\linewidth}
		\centering
		\includegraphics[width=\linewidth]{shape_variation/lamps/completed/14231_5.png}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[b]{0.25\linewidth}
		\centering
		\includegraphics[width=\linewidth]{shape_variation/lamps/completed/14231_5_2.png}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[b]{0.25\linewidth}
		\centering
		\includegraphics[width=\linewidth]{shape_variation/lamps/completed/14231_6_2.png}
    \end{subfigure}%
    \vskip\baselineskip%
    \vspace{-2.2em}
    \caption{{\bf Diversity of Object Completions}. Starting from a partial object, we show several completions using our model.
    The first two rows showcase completion results for chairs, the third and fourth for tables, and the last two rows for lamps.}
\end{figure}

==> fig/shape_generation_variable_sizes_text_guided.tex <==
\begin{figure}
    \centering
    \vskip\baselineskip%
    \vspace{-0.5em}
    \begin{subfigure}[b]{0.15\linewidth}
		\centering
		\includegraphics[trim=100 0 100 0,clip,width=\linewidth]{pasta_clip_size/chairs/completed/1382_10.png}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[b]{0.15\linewidth}
		\centering
		\includegraphics[trim=100 0 100 0,clip,width=\linewidth]{pasta_clip_size/chairs/decoder/1382_10.png}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[b]{0.15\linewidth}
		\centering
		\includegraphics[trim=100 0 100 0,clip,width=\linewidth]{pasta_clip_size/chairs/completed/44315_9_1.png}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[b]{0.15\linewidth}
		\centering
		\includegraphics[trim=100 0 100 0,clip,width=\linewidth]{pasta_clip_size/chairs/decoder/44315_9_1.png}
    \end{subfigure}%
    \vskip\baselineskip%
    \vspace{-0.5em}
    \begin{subfigure}[b]{0.15\linewidth}
		\centering
		\includegraphics[trim=100 0 100 0,clip,width=\linewidth]{pasta_clip_size/tables/completed/18831_9_1.png}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[b]{0.15\linewidth}
		\centering
		\includegraphics[trim=100 0 100 0,clip,width=\linewidth]{pasta_clip_size/tables/decoder/18831_9_1.png}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[b]{0.15\linewidth}
		\centering
		\includegraphics[trim=100 0 100 0,clip,width=\linewidth]{pasta_clip_size/tables/completed/18924_3_1.png}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[b]{0.15\linewidth}
		\centering
		\includegraphics[trim=100 0 100 0,clip,width=\linewidth]{pasta_clip_size/tables/decoder/18924_3_1.png}
    \end{subfigure}%
    \vskip\baselineskip%
    \vspace{-0.5em}
    \begin{subfigure}[b]{0.15\linewidth}
		\centering
		\includegraphics[trim=100 0 100 0,clip,width=\linewidth]{pasta_clip_size/lamps/completed/14308_3_1.png}
    \end{subfigure}%
    \begin{subfigure}[b]{0.15\linewidth}
		\centering
		\includegraphics[trim=100 0 100 0,clip,width=\linewidth]{pasta_clip_size/lamps/decoder/14308_3_1.png}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[b]{0.15\linewidth}
		\centering
		\includegraphics[trim=100 0 100 0,clip,width=\linewidth]{pasta_clip_size/lamps/completed/14589_3_1.png}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[b]{0.15\linewidth}
		\centering
		\includegraphics[trim=100 0 100 0,clip,width=\linewidth]{pasta_clip_size/lamps/decoder/14589_3_1.png}
    \end{subfigure}%
    \vskip\baselineskip%
    \vspace{-1.2em}
    \caption{{\bf Generation Results of Objects with Various Sizes}. Our model can generate shapes of different sizes.}
    \label{fig:shapenet_generations_variable_sizes}
    \vspace{-1.2em}
\end{figure}

==> fig/text_guided_generation.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.33\linewidth}
	\centering
	\includegraphics[trim={0 0 0 5cm},clip,width=\linewidth]{pasta_clip/chairs/completed/2998_9.png}
    \end{subfigure}%
     \begin{subfigure}[b]{0.33\linewidth}
	\centering
	\includegraphics[trim={0 0 0 5cm},clip,width=\linewidth]{pasta_clip/chairs/completed/42237_12.png}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[b]{0.33\linewidth}
	\centering
        \includegraphics[trim={0 0 0 5cm},clip,width=\linewidth]{pasta_clip/chairs/completed/38244_8.png}
    \end{subfigure}%
     \vskip\baselineskip%
    \vspace{-2.8em}
    \begin{subfigure}[b]{0.33\linewidth}
	\centering
	\includegraphics[trim={0 0 0 1cm},clip,width=\linewidth]{pasta_clip/chairs/decoder/2998_9.png}
    \end{subfigure}%
     \begin{subfigure}[b]{0.33\linewidth}
	\centering
	\includegraphics[trim={0 0 0 1cm},clip,width=\linewidth]{pasta_clip/chairs/decoder/42237_12.png}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[b]{0.33\linewidth}
	\centering
        \includegraphics[trim={0 0 0 1cm},clip,width=\linewidth]{pasta_clip/chairs/decoder/38244_8.png}
    \end{subfigure}%
    \vskip\baselineskip%
    \vspace{-1.5em}
    \begin{subfigure}[t]{0.32\linewidth}
	\small{\textit{A chair with four leg, one central support, one seat single surface, two arm sofa style, and one back single surface.}}
    \end{subfigure}%
    \hfill%
     \begin{subfigure}[t]{0.32\linewidth}
	\small{\textit{A chair with four leg, one bar stretcher, three runner, one seat single surface, one arm horizontal bar, two arm near vertical bar, two arm horizontal bar, two arm near vertical bar, one arm horizontal bar, and one back single surface.}}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[t]{0.32\linewidth}
        \small{\textit{A chair with four leg, two runner, one seat single surface, and one back single
        surface.}}
    \end{subfigure}%
    \vspace{-1.2em}
    \vskip\baselineskip%
    \begin{subfigure}[b]{0.33\linewidth}
	\centering
	\includegraphics[trim={0 0 0 5cm},clip,width=\linewidth]{pasta_clip/tables/completed/19307_6.png}
    \end{subfigure}%
     \begin{subfigure}[b]{0.33\linewidth}
	\centering
	\includegraphics[trim={0 0 0 5cm},clip,width=\linewidth]{pasta_clip/tables/completed/28800_14.png}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[b]{0.33\linewidth}
	\centering
        \includegraphics[trim={0 0 0 5cm},clip,width=\linewidth]{pasta_clip/tables/completed/28472_6.png}
    \end{subfigure}%
    \vskip\baselineskip%
    \vspace{-2.8em}
    \begin{subfigure}[b]{0.33\linewidth}
	\centering
	\includegraphics[trim={0 0 0 3cm},clip,width=\linewidth]{pasta_clip/tables/decoder/19307_6.png}
    \end{subfigure}%
     \begin{subfigure}[b]{0.33\linewidth}
	\centering
	\includegraphics[trim={0 0 0 3cm},clip,width=\linewidth]{pasta_clip/tables/decoder/28800_14.png}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[b]{0.33\linewidth}
	\centering
        \includegraphics[trim={0 0 0 3cm},clip,width=\linewidth]{pasta_clip/tables/decoder/28472_6.png}
    \end{subfigure}%
    \vskip\baselineskip%
    \vspace{-1.5em}
    \begin{subfigure}[t]{0.32\linewidth}
	\small{\textit{A table with two central support, two pedestal, one tabletop connector, and one board.}}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[t]{0.32\linewidth}
	\small{\textit{A table with one drawer front, one handle, one drawer front, one handle, two vertical side panel, one bottom panel, four leg, one back panel, one vertical front panel, and one board.}}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[t]{0.32\linewidth}
        \small{\textit{A table with one central support, one pedestal, one tabletop connector, one other, one board, and one tabletop frame.}}
    \end{subfigure}%
    \vskip\baselineskip%
    \vspace{-1.1em}
    \begin{subfigure}[b]{0.33\linewidth}
	\centering
	\includegraphics[trim={0 0 0 2cm},clip,width=\linewidth]{pasta_clip/lamps/completed/14370_5.png}
    \end{subfigure}%
     \begin{subfigure}[b]{0.33\linewidth}
	\centering
	\includegraphics[trim={0 0 0 2cm},clip,width=\linewidth]{pasta_clip/lamps/completed/14456_6.png}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[b]{0.33\linewidth}
	\centering
        \includegraphics[trim={0 0 0 2cm},clip,width=\linewidth]{pasta_clip/lamps/completed/16356_4.png}
    \end{subfigure}%
    \vskip\baselineskip%
    \vspace{-1.0em}
    \begin{subfigure}[b]{0.33\linewidth}
	\centering
	\includegraphics[trim={0 0 0 2cm},clip,width=\linewidth]{pasta_clip/lamps/decoder/14370_5.png}
    \end{subfigure}%
     \begin{subfigure}[b]{0.33\linewidth}
	\centering
	\includegraphics[trim={0 0 0 2cm},clip,width=\linewidth]{pasta_clip/lamps/decoder/14456_6.png}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[b]{0.33\linewidth}
	\centering
        \includegraphics[trim={0 0 0 2cm},clip,width=\linewidth]{pasta_clip/lamps/decoder/16356_4.png}
    \end{subfigure}%
    \vskip\baselineskip%
    \vspace{-1.5em}
    \begin{subfigure}[t]{0.32\linewidth}
	\small{\textit{A lamp with one lamp shade, one light bulb, one other, one chain, and one lamp base part.}}
    \end{subfigure}%
    \hfill%
     \begin{subfigure}[t]{0.32\linewidth}
	\small{\textit{A lamp with one lamp arm straight bar, one lamp shade, one light bulb, one other, one lamp base part, and one lamp body.}}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[t]{0.32\linewidth}
        \small{\textit{A lamp with one lamp shade, one light bulb, one lamp pole, and one lamp base part.}}
    \end{subfigure}%
    \vskip\baselineskip%
    \vspace{-1.2em}
    \caption{{\bf Text-guided shape generation}. Given different text descriptions 
    our model can generate plausible 3D shapes of chairs, tables, and lamps.}
    \label{fig:text_guided_generation}
\end{figure}


==> part_variations.tex <==
\input{fig/part_variations.tex}

==> tab/shapenet_generation_quantitative_all.tex <==
\begin{table}
\resizebox{\columnwidth}{!}{%
    \centering
    \begin{tabular}{l|c|c|c}
        \toprule
        \multicolumn{1}{c}{\,} & \multicolumn{1}{c}{Representation} &
        \multicolumn{1}{c}{MMD-CD ($\downarrow$)} & \multicolumn{1}{c}{COV-CD ($ \%, \uparrow$)} \\
        \midrule
        IM-Net & Implicit &  &  \\
        \midrule
        PQ-Net & Implicit Parts & 4.82 & 40.41 \\
        ATISS & Cuboids & 6.09 & 35.03 \\
        \midrule
        Ours-Parts & Cuboids & 3.82 & 51.01 \\
        Ours & Implicit & 3.24 & 50.89 \\
        \bottomrule
    \end{tabular}
    }
    \caption{{\bf Comparison with 3D Generative Models.} We train a model on
    Chairs, Tables and Lamps without any class conditioning and measure MMD-CD
    ($\downarrow$) and COV-CD ($\uparrow$).}
    \label{tab:shape_generation_quantitative_all}
    \vspace{-1.2em}
\end{table}



